Highway to HAL: Open-Sourcing the First Extendable Gate-Level Netlist Reverse Engineering Framework

Since hardware oftentimes serves as the root of trust in our modern interconnected world, malicious hardware manipulations constitute a ubiquitous threat in the context of the Internet of Things (IoT). Hardware reverse engineering is a prevalent technique to detect such manipulations. Over the last years, an active research community has significantly advanced the field of hardware reverse engineering. Notably, many open research questions regarding the extraction of functionally correct netlists from Field Programmable Gate Arrays (FPGAs) or Application Specific Integrated Circuits (ASICs) have been tackled. In order to facilitate further analysis of recovered netlists, a software framework is required, serving as the foundation for specialized algorithms. Currently, no such framework is publicly available. Therefore, we provide the first open-source gate-library agnostic framework for gate-level netlist analysis. In this positional paper, we demonstrate the workflow of our modular framework HAL on the basis of two case studies and provide profound insights on its technical foundations.

==> sections/method.tex <==
%!TEX root = ../main.tex

\section{Method}


\input{sections/hal}


\input{sections/projects}




==> sections/projects.tex <==
%!TEX root = ../main.tex
\label{sec:projects}
\subsection{Educational \& Research Material: Hardware Reverse Engineering Projects}
With our enhancements to \HAL, we were able to accompany our lectures with practical reverse engineering.
At the same time, we created a platform which enables reproducible evaluation of human processes by means of several reverse engineering projects.
The purpose of these projects is twofold.
On the one hand the projects were developed to accomplish educational goals teaching students how to practically apply various reverse engineering techniques.
On the other hand they had to be implemented as research materials to analyze human behavior in realistic hardware reverse engineering scenarios.
To investigate if the twofold purpose of the projects was successful, a pilot course has been conducted \cite{tale:2018:wiesen}.
The results of the educational evaluation showed the successful implementation of the projects as educational and research materials.
Nevertheless the analysis revealed indications for revising aspects of the single projects.
In the following the revised projects which will be used for our upcoming larger studies are presented.

\subsubsection{Project 1 - Introduction to \HAL}
An introductory project helps students to understand the various features and the functionality of \HAL.
It imparts knowledge about different gate types and their functionalities, and how \HAL can be incorporated for the reverse engineering process.
Dedicated \HAL features like automated generation Boolean functions - or rather Binary Decision Diagrams (BDDs) - to analyze the logic of gates are introduced.
Moreover applying different algorithms from graph theory, e.g., identifying strongly connected components, are included in project 1, which will support students in solving hardware reverse engineering tasks.
For that matter a simple cipher has been designed consisting of a substitution-permutation-network.

\subsubsection{Project 2 - \ac{FSM} Reverse Engineering}
In this task an \ac{FSM} circuit has to be identified in \textit{the sea of gates} and the transition logic has to be reversed.
The challenge in this task is to find the \ac{FSM} in the netlist with several thousand gates.
The task makes heavy use of novel features of \HAL, like the submodules to group parts in the netlist that belong together, as described in \Section{co::sec::hal_improvements}.
The detection of the \ac{FSM} has become more realistic by finding false positive results when it comes to identifying possible \ac{FSM} circuits.
The challenge for the students is to analyze the candidates in more detail.
Algorithms from graph theory, supporting the search, can directly be executed via \HAL plugins.
Once the component has been identified the Boolean functions of the state transition logic has to be explored in order to retrieve the states and transitions.
Live exploration can be done easily with the integrated Python interface to control \HAL (cf. \Section{co::sec::hal_improvements}).

\paragraph{What psychological insights will we gain?}
\begin{itemize}
\item First reference point of how long students need to solve the \ac{FSM} reversing task in total.
\item Analysis and description of students' mistakes during the \ac{FSM} reversing task.
\item Analysis of how much extra time effort students spent on solving mistakes.
\end{itemize}

\subsubsection{Project 3 - Obfuscated \ac{FSM}}

In \Section{asp-dac:chap:obfuscation} several obfuscation techniques to protect the control path - and thus the \ac{FSM} - have been described.
Therefore, Project 3 incorporates reversing of an \ac{FSM} based obfuscation technique named HARPOON \cite{tcad:2009:chakraborty}, as shown in \Figure{co::fig::obfsucated_fsm}.
HARPOON inserts a second \ac{FSM} (red) to protect the original \ac{FSM} (blue).
The inserted \ac{FSM} part has to be traversed in a certain way, using a specific input sequence, called the enabling key.
Every other input sequence than the enabling key will not lead to the original \ac{FSM} thus rendering the hardware design unusable for unauthorized parties.

\begin{figure}[htb]
	\centering
	\resizebox{0.7\linewidth}{!}{%
		\begin{tikzpicture}
		\tikzstyle{every state}=[fill=white,draw=black,text=black,inner sep=0pt,minimum size=17pt,circular drop shadow]

		\draw [help lines,red] (0,0) (8,5);

		% harpoon obfuscation mode
		\node[initial,state,fill=lightcoral] (sO0) at (2,2) {$s^\text{O}_0$};
		\node[state,fill=lightcoral] (sO1) at (3.5,3) {$s^\text{O}_1$};
		\node[state,fill=lightcoral] (sO2) at (5,2) {$s^\text{O}_2$};
		\node[state,fill=lightcoral] (sO3) at (3,1) {$s^\text{O}_3$};
		\node[state,fill=lightcoral] (sO4) at (4,1) {$s^\text{O}_4$};
		% harpoon authentication mode
		\node[state,fill=lightcoral] (sA0) at (1,4.5) {$s^\text{A}_0$};
		\node[state,fill=lightcoral] (sA1) at (3,4.5) {$s^\text{A}_1$};
		\node[state,fill=lightcoral] (sA2) at (5,4.5) {$s^\text{A}_2$};
		% original mode
		\node[state,fill=lightskyblue] (s0) at (7,1.25) {$s_0$};
		\node[state,fill=lightskyblue] (s1) at (7,2.25) {$s_1$};
		\node[state,fill=lightskyblue] (s2) at (7,3.25) {$s_2$};
		\node[state,fill=lightskyblue] (s3) at (7,4.25) {$s_3$};

		\path[->,>=stealth']
		(sO0) edge [above] node {$i_0$} (sO1)
		(sO0) edge (sA0)
		(sO1) edge [above] node {$i_1$} (sO2)
		(sO1) edge (sO3)
		(sO2) edge (sO4)
		(sO2) edge [anchor=center, above] node {$i_2$\ \ \ \ \ \ } (s0)
		(sO3) edge (sO0)
		(sO4) edge (sO3)
		(sO4) edge (sO0)
		(sO4) edge (sO1)
		(sO0) edge (sA0)
		(sA0) edge (sA1)
		(sA1) edge (sA2)
		(sA2) edge [bend right] (sO0)
		(s0) edge (s1)
		(s1) edge (s2)
		(s2) edge (s3)
		(s2) edge [loop left] (s2)
		(s3) edge [bend left] (s0);

		\draw [rounded corners, thick, dotted] (0.25,0.5) -- (5.5,0.5) -- (5.5,5) -- (0.25,5) -- cycle;
		\draw [rounded corners, thick, dashed] (6,0.5) -- (8,0.5) -- (8,5) -- (6,5) --cycle;

		\end{tikzpicture}
	}
	\caption{Obfuscated \ac{FSM} using HARPOON \cite{tcad:2009:chakraborty}}
	\label{co::fig::obfsucated_fsm}
\end{figure}

In this project the students need to apply the methods they learned in Project 2 in order to detect the \ac{FSM} components in a gate-level netlist.
In addition, the challenge is to circumvent the implemented obfuscation HARPOON \cite{tcad:2009:chakraborty}.
In summary, two different attacks have to be performed:
First, the states and transitions of the \ac{FSM} have to be reversed to disclose the enabling key.
Second, students will learn how to reverse the obfuscation and manipulate gate-level netlists to patch the initial state of the \ac{FSM} \cite{ches:2018:fyrbiak}.

\paragraph{What psychological insights will we gain?}
\begin{itemize}
	\item Analysis of how much time students required to solve the second \ac{FSM} reversing task in total.
	\item Comparison with reference point of total required time in Project 2.
	\item Analysis if students have solved Project 3 more efficiently (e.g., shorter solution time, less mistakes, recovering from mistakes faster).
\end{itemize}

\subsubsection{Project 4 - AES}

Project 4 combines dynamic and static netlist reverse engineering by asking the students to extract a fixed key from an AES design.
Therefore the following steps have to be performed:
First the AES S-Box has to be identified in the netlist and manipulated using \HAL in order to weaken the AES \textit{(static part)}.
Secondly, the now manipulated netlist can be used for dynamic analysis.
Due to purposeful manipulation of the netlist, simulations of the design allow for extraction of the fixed key \cite{ivsw:2017:wallat}.

\paragraph{What psychological insights will we gain?}
\begin{itemize}
	\item Analysis and description of used hardware reverse engineering strategies in the most complex task of the study.
	\item Analysis and comparison of total solution time, made mistakes and time for solving mistakes.
	\item Descriptive analysis of how students recognized patterns and structures in finding the relevant candidates for extracting the AES key.
\end{itemize}


==> sections/psychological_background.tex <==
%!TEX root = ../main.tex

\section{Psychological Background}



